Causally Consistent Normalizing Flow

Causal inconsistency arises when the underlying causal graphs captured by generative models like \textit{Normalizing Flows} (NFs) are inconsistent with those specified in causal models like \textit{Struct Causal Models} (SCMs). This inconsistency can cause unwanted issues including the unfairness problem. Prior works to achieve causal consistency inevitably compromise the expressiveness of their models by disallowing hidden layers. In this work, we introduce a new approach: \textbf{C}ausally \textbf{C}onsistent \textbf{N}ormalizing \textbf{F}low (CCNF). To the best of our knowledge, CCNF is the first causally consistent generative model that can approximate any distribution with multiple layers. CCNF relies on two novel constructs: a sequential representation of SCMs and partial causal transformations. These constructs allow CCNF to inherently maintain causal consistency without sacrificing expressiveness. CCNF can handle all forms of causal inference tasks, including interventions and counterfactuals. Through experiments, we show that CCNF outperforms current approaches in causal inference. We also empirically validate the practical utility of CCNF by applying it to real-world datasets and show how CCNF addresses challenges like unfairness effectively.

==> sections/future.tex <==
\section{Future Work}
\label{s:future}

Although \sys can generate convincing results,
it is far from perfect and can be enhanced in many directions.


\PP{DAG limitation}
A major constraint of \sys is that the causal graph must be a DAG.
Although it is a common assumption, many real-world generative processes do not adhere to this structure.
Additionally, in time-based systems like~\cite{timecasulity},
the causal relationship can fluctuate over time,
breaking the DAG assumption. 
To address that, \sys must force them to become DAG by removing some edges from the causal graph, which will negatively affect accuracy. 


One interesting direction of \sys is to relax its DAG assumption.
\sys should accommodate more complicated causal graphs like hidden confounders and non-DAG structures. 
%
To solve this problem,
we consider combining \sys with other generative models like VAE, leveraging them to analyze the complicated causal graphs.

\PP{Causal graph limitation}
Another limitation arises from the requirement of a well-defined causal graph, which is challenging to obtain in reality.
In some cases, even experts may only obtain the partial causal graph, and in other cases there exist hidden confounders whose related causalities are unable to depict.
Additionally, a well-defined causal graph is often a too strong assumption.
Users only specific causal relationships of interest, e.g. the causality between gender and admission, rather than requiring a complete causal graph.
%
\sys should be able to handle these cases more properly by supporting even incorrect causal graphs.

\iffalse
\PP{Extending applications}
While \sys primarily focuses on causal inference tasks, 
its capabilities could be extended to other domains.
For instance, \sys could be leveraged for causal discovery tasks:
If certain variables are challenging to fit, it may indicate that certain causalities are missed in the given SCM.
By incorporating appropriate causalities to the SCM, \sys could aid in causal discovery tasks. 
Overall, given its inherent causal consistency and practical data-fitting, \sys is applicable for a wide range of potential applications.
\fi

==> sections/impl.tex <==
\section{Implementation}
\label{s:impl}

\sys is implemented with the PyTorch and PyTorch Lightning framework
to maintain compatibility with the widely used
deep learning ecosystem.
%
Designed for extensibility and flexibility, \sys allows easy integration of existing and new NFs.
%
We simplify the implementation of \sys 
by standardizing that the \(T_{\theta}^{\mathbf{B}}\) 
across each layer employs the same type of NF.
%
This simplification maintains the practical universality of \sys,
and is supported by the recognized multi-layer universality of popular NF architectures such as
MAF~\cite{maf},
RealNVP~\cite{realnvp}, and
NSF~\cite{nsf}. 
%most scenarios.
%This approach is supported by 
%the multi-layer universality
%of popular NFs~\cite{maf, realnvp, nsf},
%
Note that chaining different NFs to form \(T_{\theta}^{\mathbf{B}}\) could only increase the complexity without enhancing universality.
%
\sys encounters several implementation challenges
that require non-trivial solutions
as documented below.


\PP{Initialization of CCNF}
Initialization, 
which involves setting the initial parameter values
in deep learning models, 
poses specific challenges in \sys 
beyond those typically encountered~\cite{initdef, init}. 
%Initialization denotes 
%setting the initial values of the parameters in deep learning models~\cite{initdef}.
%While initialization in general poses a challenge
%for deep learning models~\cite{init}\MX{requires citation}\QY{cited},
%\sys faces some unique initialization issues.
%
A unique issue is over-amplification and over-reduction.
%
For example, chaining ten NFs 
with an initialization function \(Y = 3X\) 
results in \(X_i = 59049U_i\) for any \(U_i\).
%
Even a slight increase in \(U_i\) can lead to 
floating-point overflow issues in \(X_i\).

To mitigate this, \sys implements constraints on 
the maximum and minimum parameter values in each NF,
following the practices in~\cite{zuko, normflows, maf}.
%
Additionally, 
if certain parameters remain excessively large
but the maximum value cannot be decreased,
\sys employs a normalization function
\(y = x / (1 + abs(x / slope))\),
where the slope is constant,
to adjust the value range accordingly as in~\cite{zuko}.
%
Both measures ensure that
\sys will avoid arithmetic overflow or underflow during training.


\PP{Modelling parameters of transformations}
\sys employs neural networks to determine 
the parameters \(\theta\) in \(T_{\theta}^{\mathbf{B}}\) 
based on the parent variables parent variables of \(\mathbf{B}\).
However, fully- or arbitrarily connected
neuron networks are inadequate for this task
due to the specific dependencies of different parts of \(\theta\)
on distinct parent variables.
%since different parts of \(\theta\) are restricted by different parent variables.
For instance, consider 
\(\theta = (\theta_1, \theta_1)\), 
\(Z_3^1 = T_{\theta_1}(U_3 | {U_1, U_2}),
Z_4^1 = T_{\theta_2}(U_4 | {U_2})\).
%
Here, \(\theta_1\) is determined by \({U_1, U_2}\) 
and \(\theta_2\) is solely determined by \({U_2}\).
%
A neuron network taking \({U_1, U_2}\) as input and 
outputting \({\theta_1, \theta_2}\) 
would incorrectly associate \(U_1\) with \(\theta_2\).
%
To resolve this, \sys employs
a methodology akin to MADE~\cite{made},
assigning specific neurons to each \(\theta_i\) and
ensuring connections only 
from relevant input neurons to the output neurons of \(\theta_i\).
%
This methodology prevents inappropriate causal linkages.


\PP{Handling discrete data}
Handling discrete data is a known challenge for NFs~\cite{nf},
and 
previous works have already proposed various solutions~\cite{nf, maf, realnvp}.
%
Similar to~\cite{causalnf}, 
\sys addresses this problem by adding a small white noise \(\epsilon\) to every discrete data.
%
The noise \(\epsilon\) is sampled from 
a normal distribution with a mean of zero 
and a small variance, e.g. \(N(0, 0.05)\).
%
This approach effectively transforms discrete distributions
into continuous ones,
which can be estimated by \sys.


\PP{Partial causality}
Partial causality refers to situations 
where only some causal connections between nodes are known,
while the complete causal graph remains elusive. 
%
To manage this,
\sys partitions the entire causal graph into distinct blocks, as inspired by~\cite{vaca, causalnf}.
%
The partition ensures that the known casualty 
only exists between blocks.
%
Within each block, causal relationships are managed by causal autoregressive flows arranged in an arbitrary sequence.
%
This strategy enables \sys to effectively handle scenarios where only partial causalities are known.

==> sections/relwk.tex <==
\section{Related Work}
\label{s:relwk}
\QY{1. compress the relwk into 1 page}

Designing GMs based on SCMs has been an active area of research, 
yielding a diverse array of models.
%
In this section,
we review previous work and
organize the discussion
based on the type of GMs involved.

\PP{NF Models}
CAREFL~\cite{carefl} represents a seminal effort
in designing NFs based on SCMs.
%
CAREFL employs an autoregressive flow, 
leveraging the analogy between autoregressive flows and causal ordering---a simplified representation of SCMs.
%
The structural similarity allows an autoregressive flow 
to effectively undertake causal inference tasks. 
%
Another significant contribution is presented in
Graphical NF~\cite{graphnf},
which illustrates the application of 
a specific NF type, RealNVP~\cite{realnvp}, 
for executing interventions and counterfactuals
within the SCMs. 
%
However, as highlighted in~\cite{causalnf},
%
for the SCMs that
are not fully connected 
(i.e., every pair of variables
are causally linked),
the causal connections within both NFs
can be superfluous,
%
thus failing to achieve causal consistency.

The state-of-the-art in causally consistent models
is represented by Causal NF~\cite{causalnf}.
%
This model achieves significant reductions 
in superfluous causal connections within NFs 
by limiting the number of hidden layers to zero. 
%
However,
as discussed in~\ref{s:intro} and
later evaluated in~\ref{s:eval},
while providing a causal consistency guarantee, 
Causal NF can only approximate distributions
for a restricted set in practice.
%
This inherent limitation underscores a trade-off
between theoretical consistency and practical utility.

\PP{VAE models}
The designing VAEs based on SCMs 
aims to embed a representation of an SCM into a VAE.
%
This can be achieved by 
transforming SCMs into a causal layer,
like~\cite{causalvae},
and incorporating it into the encoder,
or by using it to disentangle causal relationships within the latent variables, 
as seen in~\cite{deepscm, mulicave}.
%
This integration facilitates interventions and counterfactuals in VAEs.

Despite these impressive approaches,
maintaining causal consistency
between VAEs and SCMs principles 
remains a challenge.
%
VACA~\cite{vaca}
represents the state-of-the-art model that
upholds causal consistency.
%
It utilizes a Graph Neural Network (GNN)~\cite{gnn} 
to encode the specified SCM, 
leveraging on the inherent properties of GNNs
to maintain causal consistency,
particularly when the number of channels is reduced to zero. 
%
This enables VACA to effectively
perform interventions and generate counterfactuals.
%
However,
as evidenced in~\ref{s:eval}, 
constraining the GNN to zero channels limits 
the ability of VACA to accurately 
approximate the targeted distributions.

\PP{GAN Models}
Designing GANs based on SCMs is to 
incorporate interventions and counterfactuals
into the generative process of GANs.
%
CausalGAN~\cite{causalgan} and CGN~\cite{cgn},
pioneering models in this domain,
are designed to support interventions on causal variables of SCMs
in a binary setting.
%
DEAR~\cite{dear}
represents SCMs through 
a weighted adjacency matrix
which essentially encodes the latent variables.

As shown in~\cite{vaefuture}
most GAN-based models exhibit limitations in practical applications, 
researchers often find themselves needing to 
balance causal consistency with 
practical usability.
%
For instance,
while CausalGAN is designed to be causally consistent~\cite{causalgan},
its practical applicability is limited to binary attributes only~\cite{causalgan, gmcsurvey}. 
Moreover, it relies on implicit distributions, 
leaving the observational distributions unknown~\cite{causalgan, causalnf}.
%
These limitations significantly 
affect the applicability of those models and
highlight the ongoing challenges 
in integrating SCMs into GANs.

\PP{Diffusion-Based Models}
The seminal work
in the design of Diffusion-based models based on SCMs
is Diff-SCM~\cite{difscm}] and its follow-up work~\cite{healthydpm},
which is specifically engineered for counterfactual estimations.
%
Diff-SCM unifies the stochastic differential equation (SDE) framework with the SCM,
and provides a method to learn the reverse process with the SCM.
%
Furthermore,
DCM~\cite{dcm} develops distinct encoding mechanisms of SCM
to improve 
the implementation of counterfactuals
within diffusion models.

While prior works have achieved notable success
in generating counterfactuals, 
the critical issue of causal consistency
has been largely neglected.
%
As highlighted in~\cite{backcfs}, 
ensuring causal consistency is essential for a reliable counterfactual generation. 
%
Moreover, the integration of SCMs into 
diffusion-based models 
should extend 
beyond merely facilitating 
counterfactual generations.
%
Other areas, 
such as incorporating SCMs into architectures and
interpreting models,
remain unexplored.
%
These fields also require 
the establishment of causal consistency~\cite{causalnf}.
%
Therefore, it is imperative to devote
more attention and effort
to address the causal consistency problem 
in the design of diffusion models based on SCMs.






\iffalse
Integrating GMs and SCMs has been an active area of research, 
yielding a diverse array of models.
%
In this section,
we review previous work and
organize the discussion
based on the type of GMs involved.
%
Relevant GM architectures in the literature include
Normalizing Flows (NFs),
Variational Autoencoders (VAEs), 
Generative Adversarial Networks (GANs), and
Diffusion-based models.
%
Details of these foundational architectures
can be found in various studies such as~\cite{dgm4}.

\subsection{NF Mdoels}
Normalizing Flows (NFs),
as briefly discussed in~\autoref{s:intro}, 
transform simple distributions 
into more complex ones that
closely resemble the real distributions of observed data samples
through a sequence of invertible mappings~\cite{nf}.
%
Recent works have started to explore 
how SCMs can be integrated into
the design of these mappings
to encode causal mechanisms, 
as outlined in~\cite{gmcsurvey}. 
%
Such integration significantly enhances the capabilities of NFs, 
enabling them to
conduct interventions and
generate counterfactuals.

CAREFL~\cite{carefl} represents a seminal effort
in integrating SCMs into NFs.
%
CAREFL employs an autoregressive flow, 
leveraging the analogy between autoregressive flows and causal ordering---a simplified representation of SCMs.
%
The structural similarity allows an autoregressive flow 
to effectively undertake causal inference tasks. 
%
Another significant contribution is presented in
Graphical NF~\cite{graphnf},
which illustrates the application of 
a specific NF type, RealNVP~\cite{realnvp}, 
for executing interventions and counterfactuals
within the SCMs. 
%
However, as highlighted in~\cite{causalnf},
%
for the SCMs that
are not fully connected 
(i.e., every pair of variables
are causally linked),
the causal connections within both NFs
can be superfluous,
%
thus failing to achieve causal consistency.

The state-of-the-art in causally consistent models
is represented by Causal NF~\cite{causalnf}.
%
This model achieves significant reductions 
in superfluous causal connections within NFs 
by limiting the number of hidden layers to zero. 
%
However,
as discussed in~\autoref{s:intro} and
later evaluated in~\autoref{s:eval},
while providing a causal consistency guarantee, 
Causal NF can only approximate distributions
for a restricted set in practice.
%
This inherent limitation underscores a trade-off
between theoretical consistency and practical utility.


\subsection{VAE Models}
A Variational AutoEncoder (VAE)~\cite{vae} 
consists of an encoder and a decoder.
%
The encoder compresses data instances into a compact representation of latent variables, 
while the decoder reconstructs the data from the latent variables.
%
Similarly to NFs,
The integration of VAEs and SCMs 
aims to embed a representation of an SCM into a VAE.
%
This can be achieved by 
transforming SCMs into a causal layer,
like~\cite{causalvae},
and incorporating it into the encoder,
or by using it to disentangle causal relationships within the latent variables, 
as seen in~\cite{mulicave}.
%
This integration facilitates interventions and counterfactuals in VAEs.

On this train of thought,
%
DeepSCM~\cite{deepscm}
effectively employs a well-defined causal graph to
deduce counterfactual effects of latent variables in VAE, 
leveraging SCM to predict how interventions
on latent variables
might alter outcomes. 
%
CausalVAE~\cite{causalvae}
introduces a causal layer to the VAE structure,
enhancing its ability to handle interventions
by aligning the latent variables
with causal assumptions for more interpretable representations.
%
MultiCVAE~\cite{mulicave}
trains a separate CVAE~\cite{cvae}
for each variable in the causal graph of SCM, 
thus allowing for the simultaneous handling of multiple interventions and counterfactual scenarios. 

However,
despite these impressive approaches,
maintaining causal consistency
between VAEs and SCMs principles 
remains a challenge.
%
As demonstrated in~\cite{ncm},
the complex neural network that forms the foundation of both encoders and decoders
are unable to learn 
any SCM solely from training data,
let alone maintaining causal consistencies.
%
Maintaining causal consistency 
requires specially designed 
encoder and decoder architectures
tailored to each given SCM, like VACA.
%
However, applying these specially designed VAEs
to real-world scenarios are hard,
primarily because their tailored encoders
and decoders struggle to fit practical observations accurately~\cite{vaefuture}.

VACA~\cite{vaca}
represents the state-of-the-art model that
upholds causal consistency.
%
It utilizes a Graph Neural Network (GNN)~\cite{gnn} 
to encode the specified SCM, 
leveraging on the inherent properties of GNNs
to maintain causal consistency,
particularly when the number of channels is reduced to zero. 
%
This enables VACA to effectively
perform interventions and generate counterfactuals.
%
However,
as evidenced in~\autoref{s:eval}, 
constraining the GNN to zero channels limits 
the ability of VACA to accurately 
approximate the targeted distributions.

\subsection{GAN Models}
Generative Adversarial Networks (GANs)~\cite{gan}
consist of two components:
a generator and a discriminator.
%
The generator takes latent variables as input
and produces new data instances 
that are designed to resemble the training set. 
%
Meanwhile, the discriminator attempts to distinguish
between samples drawn from the training data
and samples created by the generator.
%
The integration of GANs and SCMs focuses on 
incorporating interventions and counterfactuals
into the generative process of GANs.

CausalGAN~\cite{causalgan},
a pioneering model in this domain,
is designed to support interventions on causal variables of SCMs
in a binary setting.
Both CausalGAN and a similar work CGN~\cite{cgn} enable counterfactuals
by structuring the generator to align with a specified SCM.
%
However,
both models exhibit limitations in practical applications, 
as how to use data generated 
by CausalGAN for downstream tasks
remains an unresolved issue~\cite{causalgan},
and the performance of CGN on large datasets like
ImageNet-9~\cite{imagenet} is substandard.

DEAR~\cite{dear}
represents SCMs through 
a weighted adjacency matrix
which essentially encodes the latent variables.
%
Nevertheless,
DEAR's model tends to overlook the impact of biases, 
which compromises performance as highlighted in~\cite{crlci}.
%
Additionally, PKD~\cite{pkd}
leverages pre-trained state-of-the-art generators alongside an SVM
to generate high-quality counterfactuals.
%
This approach creates data
that is suitable for causal inference.
%
However, it requires a pre-trained model
and attribute classifier, 
limiting its practical application.

Given the complexities of GANs and 
issues such as model collapse~\cite{modecollapse},
%
researchers often find themselves needing to 
balance causal consistency with 
practical usability through limitations.
%
For instance,
while CausalGAN is designed to be causally consistent~\cite{causalgan},
its practical applicability is limited to binary attributes only~\cite{causalgan, gmcsurvey}. 
Moreover, it relies on implicit distributions, 
leaving the observational distributions unknown~\cite{causalgan, causalnf}.
%
These limitations significantly 
affect the applicability of those models and
highlight the ongoing challenges 
in integrating SCMs into GANs.

%Despite these innovative approaches, 
%maintaining causal consistency 
%between the GANs architectures and SCMs
%still pose significant challenges
%given the fact that the structure of GNN 
%is complex and hard to fit.
%For instance, CausalGAN, which is the causally consistent GAN model, 
%It indicates an area for further research and development.

\subsection{Diffusion-Based Models}
A Diffusion-based model~\cite{diffusion}
generates data by stimulating the diffusion process.
%
The forward pass of diffusion involves
gradually adding noise to the data until only noise remains,
%
while the reverse pass removes noise sequentially from the data. 
%
The integration of Diffusion-based models and SCMs
primarily targets on generating counterfactuals 
based on the training set.

A seminal work
in the integration of Diffusion-based models and SCMs
is Diff-SCM~\cite{difscm}],
which is specifically engineered for counterfactual estimations.
%
Diff-SCM unifies the stochastic differential equation (SDE) framework with the SCM,
and provides a method to learn the reverse process with the SCM.
%
Building on this foundation,
work~\cite{healthydpm} evolves Diff-SCM
into the Counterfactual Diffusion Probabilistic Model (CDPM) and apply it to medical tasks, 
enabling the generation of counterfactual healthy images from patient images.
%. 
Furthermore,
DCM~\cite{dcm} develops distinct encoding mechanisms of SCM
to improve 
the implementation of counterfactuals
within diffusion models.

While prior works have achieved notable success
in generating counterfactuals, 
the critical issue of causal consistency
has been largely neglected.
%
As highlighted in~\cite{backcfs}, 
ensuring causal consistency is essential for a reliable counterfactual generation. 
%
Moreover, the integration of SCMs into 
diffusion-based models 
should extend 
beyond merely facilitating 
counterfactual generations.
%
Other areas, 
such as incorporating SCMs into architectures and
interpreting models,
remain unexplored.
%
These fields also require 
the establishment of causal consistency~\cite{causalnf}.
%
Therefore, it is imperative to devote
more attention and effort
to address the causal consistency problem 
in the integration of diffusion models and SCMs.

\boxbeg
\noindent
\textbf{Summary}:
While tremendous progress has been made
on integrating SCMs and GMs, 
several challenges remain:
\begin{enumerate}[leftmargin=*]
    \item NFs and VAEs models 
    struggle to maintain causal consistency 
    or can only do so
    by limiting the depth of hidden layers to zero.

    \item GANs models make trade-offs between
    causal consistency and
    practical usability,
    which restricts their applicability.
    
    \item Diffusion-based models
    focus predominantly on generating counterfactuals,
    overlooking the issue of causal consistency.
\end{enumerate}

\noindent
These challenges motivate us to propose \sys,
a model designed to preserve causal consistency 
without compromising accuracy.
%
This approach addresses the limitations observed in existing models
and enhances generative models' reliability and applicability in real-world issues.
%Overall, the issue of causal consistency persists across various integrations of SCMs and GMs and has not been comprehensively addressed.
%Meanwhile, \sys offers a promising approach to mitigating this challenge.
\boxend
\fi

\iffalse
`

\subsection{Causal consistency in model development}
When developing deep learning models,
especially generative models,
it is advisable to adopt a causal structure like SCM for guidance~\cite{causalgan} because SCM provides a method to control causal relationships within a generative model,
as showcased in \cite{causalvae}.
%
\MX{using terms like "good idea" is too subjective
and should not appear in academic writing.
%
An alternatives to consider:
it is advisable to adopt a causal structure like SCM for guidance
(cite a reference) because ... (briefly mention some reasons),
as showcased in XXX (mention one representative example)}
\QY{I change that expression and cite related paper.}
%
However,
many models fail to \emph{strictly enforce} causal consistency
with the chosen causal structure.
%
The inconsistent model could
deviate from the original design 
and mislead tasks like causal query~\cite{estimand}, and causal inference~\cite{deeptci} to yield unreliable results.
\MX{again, meaningless is too subjective,
please spell out the detailed consequences
using examples and references.}.
\QY{I change that in this expression and cite related papers.}

To address the causal inconsistent challenges,
\MX{try not to use words like
"this", "that", "these", "those"
in the beginning of the sentence,
%
just be specific and spell out what is the challenge.}
\QY{I change the these to causal inconsistenct}
extensive research has been conducted.
%
For instance,
VACA~\cite{vaca} adopts the GNN to encode the given SEM,
leveraging GNN's ability to keep causal consistency
when its number of channels is zero.
However, the zero channel in GNN significantly impacts its ability to approximate given distributions.
\MX{what is the drawback of VACA?}.
\QY{Add drawbacks to VACA}
%
Casual NF~\cite{causalnf} ensures causal consistency by restricting its number of hidden layers to zero as discussed previously.
%
these models provide a complete causal consistency guarantee
but can only approximate distributions of a restricted set.
\MX{is it safe to say the following?:
these models provide complete causal consistency guarantee
but can only approximate functions of a restricted set.}
\QY{Yes, that is correct. I add that sentence before}
Apart from VACA and causal NF,
other works can only partially address the issue of causal inconsistency.
\MX{the issue of?}.
\QY{Clearify the issue}
%
For instance, CAREFL~\cite{carefl} is the first work
linking NFs with causality.
However, it cannot maintain causal consistency
as it employs causal orders, rather than SCMs, to design the structure of NFs,
and causal orders cannot maintain causal consistency as proved in~\cite{causalnf}.
\MX{because?}.
\QY{Add the reason}
%
Similarly,
Graphical NF~\cite{} treats SEMs as a Bayesian network and
employs graphical conditioners to keep consistency.
\MX{any why this is not enough?}.
\QY{It is not enough, I add the reason}
%
CauF-VAE~\cite{} combines NF and VAE
\MX{i don't think VAE is mentioned yet?}
to learn causal disentangled representation and
attempts to maintain the causal consistency
by causal conditioner
\MX{any why this is not enough?}.

Overall,
while above-mentioned models incorporate causality into their designs,
they cannot guarantee casual consistency without limitations.


\subsection{Causal consistency in model training}
Causality, such as SCM,
could be used as high-level guidance when training an AI model.
\MX{again, how and why?
You need to support this claim by giving an example on
how to use SCM to do training.}
%
However, since many models
like neuron networks are regarded as black boxes,
maintaining consistency between those models and causality
becomes challenging.
\MX{I have zero idea to any of the following sentences
because I don't understand how SCM can be used in training}
%
The inconsistency makes SCM ineffective
\MX{how can it make the SCM ineffective,
the SCM is just a description of the causality,
how can a description be ineffective?} and
can lead to erroneous guidance in the training process.

Previous researchers have proposed many methods
to maintain consistency\MX{during model training?}.
%
In the theoretical part,
many researchers have tried to
build mathematical definitions and solutions of this challenge.
%
For instance,
work~\cite{} combines causal inference and deep learning,
ensuring that the learned deep learning model is
consistent with a given causal structure. 
%
Work~\cite{} demonstrates
how causal inference can be used to disentangle causal relationships
when encoding observations.
%
Work~\cite{} disentangled pose discrepancy from other variations and
to perform better face recognition. 
%
As representative learning is attracting much more attention,
I am sure related research will progress rapidly.


Although causality could be beneficial in model training, maintaining consistency is challenging and requires more effort.
\MX{What do you want to convey from this sentence?
%
As a reader, after reading this subsection, I expect a conclusion.
%
Please at least answer the following questions:
1) what is the relationship between
ensuring consistency in model development and 
ensuring consistency in model training?
%
Are they related? Are they complementary?
Do you need to do both or just one of them?
%
if you need to do just one of them,
why CCNF instead of any of the above approaches?
%
2) what do yo mean by ``maintaining'' consistency?
This seems to be a common drawback of all above-mentioned works,
you need to elaborate on this.}


\subsection{Causal consistency after model deployment}
Causal consistency,
along with its reverse, causal inconsistency,
is a powerful tool to
ensure the security of AI models and
protect them from privacy leakage post-deployment.
%
Specifically,
it means examining models through causality modeling and
finding the inconsistency from normal action.
%
An inconsistency indicates that
there exist flaws with high probability,
therefore further action is needed. 
%
For instance,
ABS~\cite{} detects backdoor attacks
by analyzing the inconsistencies in the neuron value
between benign and trojaned images.
%
SODA~\cite{} identifies potential semantic backdoors
by conducting causality analysis and
assessing the contributions of hidden neurons to the predictions.
%
For neurons
whose contributions are inconsistent with normal standards,
SODA will adjust their weights to remove the backdoor.
%
Apart from security protection,
causal inconsistency can also be applied to
protect privacy leakage.
%
ETIO~\cite{} explains membership inference (MI) attacks,
which exploit privacy leaking
through causal modeling and reasoning.

Overall, since causal consistency proves a reliable and explainable approach to protect the security and privacy of AI models, it will be applied widely in the future.
\fi



\iffalse
%
%In theory, researchers reveal the hidden connection and
%between GMs and SCMs in various aspects. 
%
%For instance, 
%work~\cite{} provides a mathematical definition of
%causal consistency in causality\MX{and
%why is this related to model training?}.
%
%And work~\cite{} links causality with neuron networks
%for causal inference tasks through causal abstractions.
%
%Work~\cite{} presents a causal mediation analysis
%for interpreting
%which parts of a model are causally implicated in its behavior.
%Practically,
%many methods,
%such as representative learning or
%causal disentangling,
%have been proposed to maintain causal consistency.

The concept of causal consistency has various definitions and applications ross different semantic frameworks,
and some of them date back to 1970s~\cite{}.

\QY{
When discussing \sys, the concept of causal consistency specifically denotes the consistency between a given causal graph and the causal graph captured by a generative model.
%
However, as a generative model, the causal inconsistency could manifest during 
model development, 
model training, 
and model deployment process.
%
Therefore we seek various strategies to ensure causal consistency in different processes.
%
Note that only ensuring causal consistency from designing, such as \sys, can solve this problem thoroughly.
%
The other two methods comprise a causal inconsistent generative model, and can only migrate the problem, which will be discussed in the following.
%
Therefore, ensuring causal consistency in design is sufficient for generative models.
}

\MX{Honestly I did not quite get the meaning of this paragraph.}

\MX{When I read the sentence:
"The concept of causal consistency has various definitions
and applications...",
my expectation is:
%
okay the authors are trying to list the
definitions and applications and
nail down to a specific one (relevant to this paper).
%
But this is not the case.}
\QY{The origin writing is particularly misleading. In the new paragraph, I nail down the causal consistency and introduce from that point.}

\MX{When I read the sentence:
"could be applied to different stages of the AI's lifecycle",
%
I am totally confused as:
1) what is AI's lifecycle? and who defines such lifecycle?
and more importantly, 2) why would I need to care about this?
%
What is the purpose that you introduce the lifecycle?
You may say this is to provide a systematic way of organizing things,
but why using the lifecycle as a way to organize this?}
\QY{To avoid this, I remove the concept of AI lifecycle. I originally wanted to employ it in a systematic way, but here I changed the expression.}

\MX{Even worse,
this lifecycle thing puts a lot of questions in my head.
%
Let's say, if you want to ensure causal consistency,
do you need to ensure consistency at all stages?
%
Clearly CCNF is only targeting the model development stage,
so what is the downside of not enforcing causality in other stages?
Do that compromise CCNF's claim?}
\QY{I clarify this point in the new paragraph and remove the related misleading concept.}

\MX{Last but not least,
I would suggest that don't use big words such as AI,
just say machine learning or neural networks,
in academic writing,
the more specific (or the more precise) the better.}
\QY{Yes, I change all the AI to generative models here and after.}





\PP{Incorporating SCM into the generation}
Rather than modifying GANs, 
alternative works leverage GANs 
to implement interventions of given SCMs.
%
For instance, 
GenInt~\cite{genint} enhances the robustness of visual classifiers 
by a conditional GAN (cGAN).
It eliminates spurious correlations through an SCM and
improves the performance of the classifiers.
work~\cite{genint3d} extends the approach in GenInt to the 3D field.
%
PKD~\cite{pkd} uses pre-trained state-of-the-art generators to generate 
high-quality counterfactuals for knowledge extrapolation.
%
However, all the models do not take causal consistency into the design,
therefore the causal inconsistent problem could emerge in their models.
\fi
